Trajectory and Sway Prediction Towards Fall Prevention

Falls are the leading cause of fatal and non-fatal injuries, particularly for older persons. Imbalance can result from the body's internal causes (illness), or external causes (active or passive perturbation). Active perturbation results from applying an external force to a person, while passive perturbation results from human motion interacting with a static obstacle. This work proposes a metric that allows for the monitoring of the person's torso and its correlation to active and passive perturbations. We show that large changes in the torso sway can be strongly correlated to active perturbations. We also show that we can reasonably predict the future path and expected change in torso sway by conditioning the expected path and torso sway on the past trajectory, torso motion, and the surrounding scene. This could have direct future applications to fall prevention. Results demonstrate that the torso sway is strongly correlated with perturbations. And our model is able to make use of the visual cues presented in the panorama and condition the prediction accordingly.

==> Sections/3RelatedWork.tex <==
\section{Related Work}

(Perhaps this should be moved to introduction) Before we dive into the related work, it is important to make a distinction between fall detection and fall prediction. Fall detection happens after the fall, and it has been a relatively well studied area that made its way to the wearable smart devices several years ago. While fall prediction happens before the actual event, it offers a chance to intervene and neutralize the risk. Current attempts to predict falling includes ...

\todo[inline]{Find references that relates to:(fusing imu data[1],pressure sensing insoles[2], test effectiveness putting sensors at different locations[2], external pose tracking[4]) 

I have those for now: \cite{chen_reliable_2010}, \cite{howcroft_prospective_2017}, \cite{preis_gait_nodate}, \cite{oday_assessing_2022}

}. 

They are either too focused on the intrinsic factors, or the technique is inapplicable to the real world scenario. \todo[inline]{And then elaborate on this a little more}

Fall prediction is naturally a multi-modal problem, there are 4 major contributing factors: Biological, Environmental, Behavioral, and Demographic. \cite{rajagopalan_fall_2017} Majority of the past work focused on the Biological factors such as gait disturbances and postural instability. \todo[inline]{(insert works that predict/detect using biological factors), should be a easy look in in the paper above} We would like to argue that the extrinsic environmental factors can be equally important when it comes to fall prediction. 

% \todo[inline]{As a reference, here is the diagram they are using:
% \begin{figure}[H]
%     \centering
%     \includegraphics[width = \textwidth]{Figures/S3factors.png}
%     \caption{}
%     \label{img:concept}
% \end{figure}
% }
% perhaps a paragraph to discuss stability metrics
center of gravity as alternative stability/balance metric

==> Sections/Drafts/intro_draft1_ken_michael.tex <==
INTRODUCTION}

% Focus: design choices, why did you design the work like this

Falling has been a leading cause of injury and hospitalization in older adults. There are many works tries to detect the fall after the occurrence. However, such post-fall detection offers little help to prevent the injury. In this work, we hope to create a wearable device in conjunction with a suitable network model to: actively monitor the surrounding, predict the future gait and stability of the user conditioned on the environment, and issue alert when the fall is imminent.


\begin{figure}[t!]
    \centering
    \includegraphics[width = 0.5\textwidth]{Figures/S2concept.png}
    \caption{System Concept: We present a system capable of predicting future path, velocity and torso sway conditioned on the environment and past motion of the wearer. The ability to predict significant change in the wearer's sway is correlated with passive or active perturbations that may lead to instability. The pose of the wearer is detected through visual inertial odometry from a camera and inertial measurement unit mounted on the torso. The environment is processed into a depth panorama image for a consistent dimension representation in neural network use. The sway is found by projecting the torso's upward facing z-axis into the transverse plane aligned with world z-axis, then tracking the variance of this projected vector over a sliding window. Large change in the sway variance ellipsoid is correlated with active and passive perturbations.}
    \label{img:concept}
\end{figure}

Previous work on gait and stability has largely focused on metrics derived from classical models of walking, such as an inverted pendulum \cite{kuo2005energetic, hof2005condition}. 
One classical metric for gait stability is the Margin of Stability \cite{hof2005condition}, which has also been used to quantify recovery responses to gait perturbations \cite{roeles2018gait}. While these classical models serve as a useful framework for understanding gait and balance, their simplified structure inherently limits their ability to explain some of the more complex actions generated by the human nervous system. Data-driven methods are an effective tool to explain some of the more complex, varied aspects of human gait. With the advent of improved wearable sensors, compute, and learning algorithms, data-driven approaches have been gaining traction in recent years. Several studies have shown the efficacy of using a machine learning (ML) approach with worn inertial measurement units (IMU)s to achieve high accuracy in detecting near-fall events from disturbances such as stumbling over uneven terrain \cite{hartog2021stumblemeter, aziz2012distinguishing, choi2011study}. 
While these approaches show strong results in gait event detection, they rely on population-specific training data consisting of gait disturbances, steady-state walking, and other common activities of daily life, such as sitting, standing, and lying down. The effectiveness of a learned model is largely determined by the quality of its training data, and given the large variability in human gait, especially among various patient populations at elevated risk of falling, minimizing pathology-specific training data is essential to the utility of the gait disturbance detector. 
For this reason, in the part of our system identifying changes in user gait, we opted for a strategy to detect a pattern in gait from the current user and detect deviations from that pattern, rather than rely on aggregated, population-specific training data. 
While some methods have used wearable sensors and simple acceleration threshold algorithms to detect a fall and intervene \cite{tamura2009wearable, chan2006human}, their fall detection algorithms are either not fully described or rely on the person to achieve complete free-fall before intervening, thus mitigating injury but still allowing the fall to occur. This method suffers from two aspects, one it requires the person have already entered a state that is unrecoverable from a fall, and second, ignores precursor cues of torso motion that may have been strong indicators of imbalance. 
To this end we propose Torso Sway Variance, which monitors the natural sway of the person as they walk. By tracking the projection of their torso z-axis into the world transverse plane, we calculate the variance in their torso sway over a sliding window, as shown in fig. \ref{img:concept}. This variance ellipse in the transverse plane is different for each individual, but the change in the ellipse area has strong correlation to perturbation which we show in fig. \ref{img:DsigZ}
% To our knowledge, our system is the first approach to detect gait disturbances that could lead to a fall with sufficient lead time to prevent the fall without relying on aggregated, patient-specific training data.




% Previous work on gait and stability has largely focused on metrics derived from classical models of walking, such as an inverted pendulum \cite{kuo2005energetic, hof2005condition}. One popular metric for gait stability is the Margin of Stability (MoS) \cite{hof2005condition}, which uses  knowledge of the body's base of support (BoS), center of mass (CoM), and the natural frequency of the torso and leg modelled as an inverted pendulum. The BoS is defined as the region between and beneath the feet where the center of pressure can move. The Margin of Stability is calculated by first propagating the center of mass forward in time using the natural frequency, known as the extrapolated center of mass (XCoM). The distance between the XCoM and the BoS is the Margin of Stability. In addition to being used to quantify overall stability, MoS has been shown to change in the steps immediately following various types of perturbations \cite{roeles2018gait}. 

% \todo[inline]{Michael points on gait perturbation and known disturbance metrics}

% [Contributions FYI]
%   1.(Representation) Proposed a novel way to effectively and universally represent the surrounding environment \\
%   2.(Prediction) Demonstrated a multimodal approach to state prediction task \\
%       - Predict future stability and pose, conditioned on the environment and past trajectory \\
%   3.(Stability) Relation between ground features and [stability] (no learning involved) (maybe replace stability with z projection) \\
%   4.(System) Realworld dataset and system integration \\


\textcolor{red}{list of refs:}  \nocite{*}.

==> glossary.tex <==
% Latex glossaries: https://www.overleaf.com/learn/latex/glossaries
%example: \acrshort{lfd} or \acrfull{lfd}; or \gls{lfd}. As we will not want to list the glossary, please use the asterisk: \gls*{--}; And if you use \gls{}, it will put the full acronym the first time it is called, then the shortened version there-after. \acrfull{} will force full form
\usepackage[acronym,nomain,nonumberlist]{glossaries}
\makeglossaries
%
%Example: \newacronym{name_you_call}{Short_form}{Full_form} %then just \gls{name_you_call}, and if you want to restate the full: \acrfull{name_you_call}
% To get plural \glspl{name_you_call}


\newacronym{CoP}{CoP}{Center of Pressure}
\newacronym{CoM}{CoM}{Center of Mass}
\newacronym{MoS}{MoS}{Margin of Stability}
\newacronym{IMU}{IMU}{Inertial Measurement Unit}
\newacronym{VIO}{VIO}{Visual Inertial Odometry}
\newacronym{LSTM}{LSTM}{Long-Short Term Memory Network}
\newacronym{GRU}{GRU}{Gated Recurrent Unit}
\newacronym{VAE}{VAE}{Variational AutoEncoder}
\newacronym{RNN}{RNN}{Recurrent Neural Network}
\newacronym{MLP}{MLP}{Multi-Layer Perceptron Network}
\newacronym{CNN}{CNN}{Convolutional Neural Network}

% \newacronym[glslongpluralkey={Brain-Computer Interfaces}]{BCI}{BCI}{Brain-Computer Interface}


==> prep_notes/kennedy_prep_notes.tex <==
Refs: 
\begin{itemize}
\item \cite{prietoMeasuresPosturalSteadiness1996a} is an anchor paper for measures of postural steadiness, particularly, by using the center of pressure (COP) (requires a force platform), the area enclosed by the motion of the COP during a gait cycle (triangles formed) is the sway area
\item The paper \cite{hufschmidtMethodsParametersBody1980} is the original, the original paper in 1980 on sway params, took center of pressure (COP or COF (force)) from the feet on a platform, and tracked the motion of the COP. the sway area SA was one parameter found by taking the average position over 37 steps and for two consecutive positions, making a triangle between the consecutive pts Pi, Pi+1 and the arithmetic mean point (AMP). This and all methods like it require a) force plate b) shifted weight motion which could be accomplished through many body motion types (not clear indicators of stability: e.g. shifting weight while staying upright).
\item \cite{maBalanceImprovementEffects2016} Good review article on biofeedback systems for balance improvement; provides good future objectives including (dynamic balance, smaller sensor suite that works outdoors, enhancing devices for commercial market (e.g. phone))
\item \cite{cellaDevelopmentValidationRobotic2020} (not strong ref), Uses robot to predict likelihood of long-term fall risk. This is done by taking their clinical history/factors and using a robot called Hunova that measures a humans metrics as they stand on the device (static balance), this had about 70% accuracy of predicting a fall within a year.
\item wearable sensor for gait classification (standing/walking/steps) and characteristics monitoring \cite{singhIntentionDetectionGait2019}; no prevention, just data aggregation
\item \cite{linReliabilityCOPbasedPostural2008} discusses reliability of sway measures, best were mean velocity and sway area (79\% reliable within a day for younger ppl and 92\% reliable within a day for older people; for btw day older ppl rate stayed comparable, but younger dropped about 5-7\%); mean velocity here is avg velocity of COP in the AP (anterior-posterior front/back) direction.
\item \cite{jiangElderlyFallRisk2011} Paper uses phone with IMU mounted on center front waist to monitor gait. by looking at a window of accelerometer data passed through a dynamic time warping algorithm on accelerometer motion for front/back for symmetry and up/down (vertical) for stability. the DTW indices values indicate *regularity* of the gait which is detected
\item  \cite{zhangRecentDevelopmentHuman2022} covers modes of data collection (external and body attached) as well as gait prediction methods and associated learning architectures. provides table II of motion prediction methods
\item Methods of motion prediction (from \cite{zhangRecentDevelopmentHuman2022}) include full body prediction (e.g for pedestrians) (\cite{duBioLSTMBiomechanicallyInspired2019}, \cite{sangHumanMotionPrediction2020}, \cite{martinezHumanMotionPrediction2017}, \cite{guoHumanMotionPrediction2019},\cite{coronaContextawareHumanMotion2020}, ); and just general motion (traj++ does bounding box motion \cite{salzmannTrajectronDynamicallyFeasibleTrajectory2020} 
\end{itemize}

